Local SGD Optimizes Overparameterized Neural Networks in Polynomial Time

In this paper we prove that Local (S)GD (or FedAvg) can optimize deep neural networks with Rectified Linear Unit (ReLU) activation function in polynomial time. Despite the established convergence theory of Local SGD on optimizing general smooth functions in communication-efficient distributed optimization, its convergence on non-smooth ReLU networks still eludes full theoretical understanding. The key property used in many Local SGD analysis on smooth function is gradient Lipschitzness, so that the gradient on local models will not drift far away from that on averaged model. However, this decent property does not hold in networks with non-smooth ReLU activation function. We show that, even though ReLU network does not admit gradient Lipschitzness property, the difference between gradients on local models and average model will not change too much, under the dynamics of Local SGD. We validate our theoretical results via extensive experiments. This work is the first to show the convergence of Local SGD on non-smooth functions, and will shed lights on the optimization theory of federated training of deep neural networks.

==> checklist.tex <==
\section*{Checklist}
 

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec: discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{It is a pure theory paper and it will not have any potential negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec: convergence}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
   \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}

\end{enumerate}

==> command.tex <==
\usepackage{epsf}
%\usepackage{fancyheadings}
\usepackage{graphics}
%\usepackage{graphicx}

%\usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{psfrag}

\usepackage{color}

\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{fdsymbol}
%\usepackage[linesnumbered, ruled, vlined]{algorithm2e}
%\usepackage{ntheorem}

%\usepackage[backend=bibtex,firstinits=true]{biblatex}

%\setlength{\textwidth}{\paperwidth}
%\addtolength{\textwidth}{-6cm}
%\setlength{\textheight}{\paperheight}
%\addtolength{\textheight}{-4cm}
%\addtolength{\textheight}{-1.1\headheight}
%\addtolength{\textheight}{-\headsep}
%\addtolength{\textheight}{-\footskip}
%\setlength{\oddsidemargin}{0.5cm}
%\setlength{\evensidemargin}{0.5cm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MACROS HERE

%%%%%%%
%\theoremstyle{plain}

% {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% throughout the paper

%\theoremprework{\begin{minipage}{\textwidth}}
%\theorempostwork{\end{minipage}}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{assumption}{Assumption}
\newtheorem{exmp}{Example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
%\newlength{\widebarargwidth}
%\newlength{\widebarargheight}
%\newlength{\widebarargdepth}
%\DeclareRobustCommand{\widebar}[1]{%
%  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
%  \settoheight{\widebarargheight}{\ensuremath{#1}}%
%  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
%  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
%  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
%  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
%    \hspace{0.3\widebarargdepth}%
%    \addtolength{\widebarargheight}{0.3ex}%
%    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
%  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced 
%%% and indents them to set them off more from the text.
%\makeatletter
%\long\def\@makecaption#1#2{
%        \vskip 0.8ex
%        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
%        \parindent 1.5em  %% How can we use the global value of this???
%        \dimen0=\hsize
%        \advance\dimen0 by -3em
%        \ifdim \wd\@tempboxa >\dimen0
%                \hbox to \hsize{
%                        \parindent 0em
%                        \hfil 
%                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
%                                {\bf #1.} #2
%                                %%\unhbox\@tempboxa
%                                } 
%                        \hfil}
%        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
%        \fi
%        }
%\makeatother

\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\ordertil}{\ensuremath{\widetilde{\order}}}
\newcommand{\w}{\bm{w}}
\newcommand{\al}{\bm{\alpha}}

%% COMMENTING commands

\long\def\comment#1{}

\newcommand{\bm}[1]{\boldsymbol{#1}}
\newcommand{\llVert}{\left\lVert}
\newcommand{\rrVert}{\right\rVert}
\newcommand{\bit}[1]{\boldsymbol{#1}}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\mjwcomment}[1]{{\bf{{\red{{MJW --- #1}}}}}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\mycomment}[1]{{\bf{{\blue{{AP --- #1}}}}}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\vidyacomment}[1]{{\bf{{\green{{VM --- #1}}}}}}
\newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\cmcomment}[1]{{\bf{{\cyan{{CM --- #1}}}}}}

% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{|\!|\!| #1 | \! | \!|_{{#2}}}
\newcommand{\vecnorm}[2]{\| #1\|_{#2}}

\newcommand{\defn}{:\,=}

%Hamming metric
\newcommand{\dH}{\mathsf{d}_{\mathsf{H}} }

\newcommand{\id}{\mathsf{id}}

\newcommand{\KT}{\mathsf{KT}}

\newcommand{\dimone}{n_1}
\newcommand{\dimtwo}{n_2}
\newcommand{\maxdimonetwo}{\left(\dimone \lor \dimtwo \right)}

\newcommand{\Aone}{{\bf C1} }
\newcommand{\Atwo}{{\bf C2} }

\newcommand{\csst}{\mathbb{C}_{\mathsf{SST}}}
\newcommand{\cdiff}{\mathbb{C}_{\mathsf{DIFF}}}
\newcommand{\Cpara}{\mathbb{C}_{\mathsf{PARA}}}
\newcommand{\Cbiso}{\mathbb{C}_{\mathsf{BISO}}}
\newcommand{\Cns}{\mathbb{C}_{\mathsf{NS}}}
\newcommand{\Cnspi}{M_{\mathsf{NS}, \pi}}
\newcommand{\Mns}{M_{\mathsf{NS}}}
\newcommand{\Cnspihat}{M_{\mathsf{NS}, \pihat}}

\newcommand{\sk}{S_k}
\newcommand{\bl}{\mathsf{bl}}

\newcommand{\bltilde}{\widetilde{\mathsf{bl}}}
\newcommand{\Bl}{\mathsf{B}}
\newcommand{\Rw}{\mathsf{R}}

\newcommand{\tauhat}{\widehat{\tau}}
\newcommand{\Chatt}{\widehat{C}_t}

\newcommand{\rhat}{\widehat{\mathsf{r}}}
\newcommand{\rspace}{\mathsf{r}}

\newcommand{\elts}{\mathsf{s}}
\newcommand{\Ntilde}{\widetilde{N}}

\newcommand{\lambdahat}{\widehat{\lambda}}

\newcommand{\Cmodel}{\mathbb{C}}

\newcommand{\pobs}{p_{\mathsf{obs}}}

\newcommand{\sgn}{\mathsf{sgn}}

\newcommand{\nucnorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{nuc}}}}}
\newcommand{\fronorm}[1]{\ensuremath{\matsnorm{#1}{\footnotesize{\mbox{fro}}}}}
\newcommand{\opnorm}[1]{\ensuremath{\matsnorm{#1}{\tiny{\mbox{op}}}}}


% Inner product
\newcommand{\inprod}[2]{\ensuremath{\langle #1 , \, #2 \rangle}}

% Kullback-Leibler
\newcommand{\kull}[2]{\ensuremath{D(#1\; \| \; #2)}}

% Probability
\newcommand{\E}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}

% Observations, dimension etc.
\newcommand{\numobs}{\ensuremath{n}}
\newcommand{\usedim}{\ensuremath{d}}

\newcommand{\Comp}{\ensuremath{C}}

\newcommand{\Mrisk}{\ensuremath{\mathcal{M}}}
\newcommand{\Erisk}{\ensuremath{\mathcal{E}}}
\newcommand{\Arisk}{\ensuremath{\mathcal{A}}}

\newcommand{\diam}{\ensuremath{\mathsf{diam}}}
%Numbering
\newcommand{\1}{\ensuremath{{\sf (i)}}}
\newcommand{\2}{\ensuremath{{\sf (ii)}}}
\newcommand{\3}{\ensuremath{{\sf (iii)}}}
\newcommand{\4}{\ensuremath{{\sf (iv)}}}
\newcommand{\5}{\ensuremath{{\sf (v)}}}
%Eigenvector / eigenvalue related notation
\newcommand{\eig}[1]{\ensuremath{\lambda_{#1}}}
\newcommand{\eigmax}{\ensuremath{\eig{\max}}}
\newcommand{\eigmin}{\ensuremath{\eig{\min}}}

\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\abs}{abs}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\child}{child}
\DeclareMathOperator{\parent}{parent}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{{\sf rank}}
\DeclareMathOperator{\card}{{\sf card}}
\DeclareMathOperator{\range}{{\sf range}}
\DeclareMathOperator{\toeplitz}{toeplitz}


% 
\newcommand{\NORMAL}{\ensuremath{\mathcal{N}}}
\newcommand{\BER}{\ensuremath{\mbox{\sf Ber}}}
\newcommand{\BIN}{\ensuremath{\mbox{\sf Bin}}}
\newcommand{\Hyp}{\ensuremath{\mbox{\sf Hyp}}}

\newcommand{\Xspace}{\ensuremath{\mathcal{X}}}
\newcommand{\Yspace}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zspace}{\ensuremath{\mathcal{Z}}}
\newcommand{\Fspace}{\ensuremath{\mathcal{F}}}
\newcommand{\Ospace}{\ensuremath{\mathcal{O}}}

\newcommand{\Bupper}{\ensuremath{\overline{B}}}
\newcommand{\Blower}{\ensuremath{\underline{B}}}
% Basic statistics notation
% True parameter
\newcommand{\thetastar}{\ensuremath{\theta^*}}
% Estimate one
\newcommand{\thetahat}{\ensuremath{\widehat{\theta}}}

\newcommand{\xhat}{\ensuremath{\widehat{x}}}
\newcommand{\Deltahat}{\ensuremath{\widehat{\Delta}}}

\newcommand{\Deltatilde}{\ensuremath{\widetilde{\Delta}}}
\newcommand{\udiff}{\ensuremath{\mathbb{U}^{{\sf diff}}_m(A)}}
\newcommand{\Xhat}{\ensuremath{\widehat{X}}}
\newcommand{\Yhat}{\ensuremath{\widehat{Y}}}
\newcommand{\Ytilde}{\ensuremath{\widetilde{Y}}}
\newcommand{\Mhat}{\ensuremath{\widehat{M}}}
\newcommand{\Mstar}{\ensuremath{M^*}}
\newcommand{\Mtilde}{\ensuremath{\widetilde{M}}}
\newcommand{\bhat}{\ensuremath{\widehat{b}}}
\newcommand{\Mhatasp}{\ensuremath{\widehat{M}}_{\mathsf{ASP}}}
\newcommand{\ASP}{\ensuremath{\mathsf{ASP}}}

\newcommand{\CRL}{\ensuremath{\mathsf{CRL}}}

\newcommand{\Mhattds}{\ensuremath{\widehat{M}}_{{\sf TDS}}}

\newcommand{\Mhatod}{\ensuremath{\widehat{M}}_{{\sf 1D}}}
\newcommand{\Mhatls}{\ensuremath{\widehat{M}}_{{\sf LS}}}
\newcommand{\Mhatpermr}{\ensuremath{\widehat{M}}_{{\sf permr}}}

\newcommand{\BAP}{\ensuremath{\mathsf{BAP}}}
\newcommand{\agg}{\ensuremath{\mathsf{Agg}}}
\newcommand{\Mhatbap}{\ensuremath{\widehat{M}}_{\mathsf{BAP}}}

\newcommand{\Btilde}{\ensuremath{\widetilde{B}}}

\newcommand{\xhatml}{\ensuremath{\widehat{x}_{{\sf ML}}}}
\newcommand{\Xhatml}{\ensuremath{\widehat{X}_{{\sf ML}}}}
% Estimate two
\newcommand{\thetatil}{\ensuremath{\widetilde{\theta}}}

\newcommand{\gt}{\ensuremath{\widetilde{g}}}

\newcommand{\yvec}{\ensuremath{y}}
\newcommand{\Xmat}{\ensuremath{X}}

\newcommand{\widgraph}[2]{\includegraphics[keepaspectratio,width=#1]{#2}}


%Problem-specific notation
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
\newcommand{\real}{\ensuremath{\mathbb{R}}}

\newcommand{\Pihat}{\ensuremath{\widehat{\Pi}}}
\newcommand{\pihat}{\ensuremath{\widehat{\pi}}}
\newcommand{\pihatborda}{\ensuremath{\widehat{\pi}_{\sf bor}}}
\newcommand{\pihatpre}{\ensuremath{\widehat{\pi}_{\sf pre}}}
%\newcommand{\pihatref}{\ensuremath{\widehat{\pi}_{\sf ref}}}
\newcommand{\pihattds}{\ensuremath{\widehat{\pi}_{\sf tds}}}
\newcommand{\pihatoned}{\ensuremath{\widehat{\pi}_{{\sf 1D}}}}
\newcommand{\pihatftds}{\ensuremath{\widehat{\pi}_{{\sf tds}}}}
\newcommand{\sigmahat}{\ensuremath{\widehat{\sigma}}}
\newcommand{\Sigmahat}{\ensuremath{\widehat{\Sigma}}}
\newcommand{\sigmahatborda}{\ensuremath{\widehat{\sigma}_{\sf bor}}}
%\newcommand{\sigmahatref}{\ensuremath{\widehat{\sigma}_{\sf ref}}}
\newcommand{\sigmahattds}{\ensuremath{\widehat{\sigma}_{\sf tds}}}
\newcommand{\sigmahatftds}{\ensuremath{\widehat{\sigma}_{\sf tds}}}
\newcommand{\sigmahatpre}{\ensuremath{\widehat{\sigma}_{\sf pre}}}

\newcommand{\pihatasp}{\ensuremath{\widehat{\pi}_{\mathsf{ASP}}}}
\newcommand{\Pihatml}{\ensuremath{\widehat{\Pi}_{{\sf ML}}}}
\newcommand{\Pitil}{\ensuremath{\widetilde{\Pi}}}

\newcommand{\Projpi}{\ensuremath{P_{\Pi}}}
\newcommand{\Projorthpi}{\ensuremath{P_{\Pi}^{\perp}}}
\newcommand{\Projorthpistar}{\ensuremath{P_{\Pi^*}^{\perp}}}

\newcommand{\hballpi}{\ensuremath{\mathbb{B}^{\sf H}_\Pi}}
\newcommand{\hballpistar}{\ensuremath{\mathbb{B}_{\sf H}}}
%\newcommand{\hballpistar}{\ensuremath{\mathcal{P}_n}}
\newcommand{\SNR}{\ensuremath{\frac{\|x^*\|_2^2}{\sigma^2}}}
\newcommand{\col}{\ensuremath{{\sf col}}}
\newcommand{\row}{\ensuremath{{\sf row}}}
\newcommand{\Pn}{\ensuremath{\mathcal{P}_n}}

\newcommand{\EE}{\ensuremath{\mathbb{E}}}
%changed to probability of error
\newcommand{\Rpihat}{\ensuremath{\Pr\{ \Pihat \neq \Pi^* \} }}

\newcommand{\Rpihatml}{\ensuremath{\Pr\{ \Pihatml \neq \Pi^* \}}}
\newcommand{\BigO}{\ensuremath{\mathcal{O}}}


\newcommand{\numitems}{\ensuremath{n}}

% commands that CM changed/introduced
\newcommand{\symgp}{\mathfrak{S}}
\newcommand{\vars}{\zeta}
\newcommand{\maxvarone}{(\vars^2 \lor 1)}
\newcommand{\varplusone}{(\vars + 1)}
\newcommand{\allones}{\mathbf{e}}
\newcommand{\bfone}{\mathbf{1}}
\DeclareMathOperator{\trace}{\mathsf{tr}}
\DeclareMathOperator{\Poi}{\mathsf{Poi}}
\DeclareMathOperator{\var}{\mathsf{var}}
\DeclarePairedDelimiter\tv{\mathsf{tv}(}{)}

%\newcommand{\Cperm}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{r},\mathsf{c}}}
\newcommand{\Cperm}{\mathbb{C}_{\mathsf{Perm}}}
%\newcommand{\Cpermr}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{r}}}
%\newcommand{\Cpermc}{\mathbb{C}_{\mathsf{Perm}}^{\mathsf{c}}}
\newcommand{\Cskew}{\mathbb{C}_{\mathsf{skew}}}

\newcommand{\tds}{{\sf TDS}}

\newcommand{\Ypoi}{Y_{\sf Poi}}
%\newcommand{\Ysortcol}{Y_{\sf sortcol}}
%\newcommand{\Ysortrow}{Y_{\sf sortrow}}

\newcommand{\BL}{\mathsf{BL}}

\newcommand{\Mps}{M_{\pi, \sigma}}
\newcommand{\Dps}{\Delta_{\pi, \sigma}}
\newcommand{\Cdiffps}{\cdiff(\pi, \sigma)}
\newcommand{\Zps}{Z_{\pi, \sigma}}
\newcommand{\Ztil}{\Zps}
\newcommand{\At}{\mathcal{A}_t}
\newcommand{\Wtil}{\widetilde{W}}
\newcommand{\cE}{\mathcal{E}}

\newcommand{\bllarge}{\mathsf{BL}^{\mathbb{L}}}
\newcommand{\blsmall}{\mathsf{BL}^{\mathbb{S}}}
%\newcommand{\blunion}{\cup \mathsf{bl}}
%\newcommand{\bllargeunion}{\cup \bllarge}
%\newcommand{\blsmallunion}{\cup \blsmall}
\newcommand{\blone}{\BL^{(1)}}
\newcommand{\bltwo}{\BL^{(2)}}
%\newcommand{\blthree}{\BL^{(3)}}
\newcommand{\blt}{\BL^{(t)}}
%\newcommand{\bltp}{\BL^{(t')}}

\newcommand{\blocksize}{\dimtwo \sqrt{\frac{\dimone}{N} \log (\dimone \dimtwo) }}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> impact.tex <==
\section*{Broader Impact}
This work advocates a distributionally robust algorithm for federated learning. The algorithmic solution is designed to preserve the privacy of users, while trains a high quality model. The proposed algorithm tries to minimize the maximum loss among distributions (clients' data). Hence, we can ensure that even if the data distribution among users is highly heterogeneous the trained model is reasonably good for everyone, and not benefiting only a group of clients. This will ensure the fairness in training a global model with respect to every user, and it is vitally important for critical decision making systems such as healthcare. In such a scenario, the model learned by simple algorithms such as FedAvg would have an inconsistent performance over different distributions, which is not acceptable. However, the resulting model from our algorithm will have robust performance over different distributions it has been trained on.
